Masked Collaborative Contrast for Weakly Supervised Semantic Segmentation

This study introduces an efficacious approach, Masked Collaborative Contrast (MCC), to highlight semantic regions in weakly supervised semantic segmentation. MCC adroitly draws inspiration from masked image modeling and contrastive learning to devise a novel framework that induces keys to contract toward semantic regions. Unlike prevalent techniques that directly eradicate patch regions in the input image when generating masks, we scrutinize the neighborhood relations of patch tokens by exploring masks considering keys on the affinity matrix. Moreover, we generate positive and negative samples in contrastive learning by utilizing the masked local output and contrasting it with the global output. Elaborate experiments on commonly employed datasets evidences that the proposed MCC mechanism effectively aligns global and local perspectives within the image, attaining impressive performance. The source code is available at \url{https://github.com/fwu11/MCC}.

==> sections/fig_abl_mask.tex <==
\begin{figure}
\centering
\includegraphics[width=0.45\textwidth, height=0.2\textwidth]{images/abl_1.pdf}
\caption{Ablation Study on Random Masking under varying the masking ratios and scales. The results are reported in the format of Pesudo/Seg. from VOC \emph{val} set in terms of mIoU($\%$).}
\label{fig:abl_mask}
\end{figure}

==> sections/fig_coco_cam_results.tex <==
\begin{figure*}[!htbp]
\centering
\includegraphics[width=0.85\linewidth,height=0.4\linewidth]{images/coco_cam_results.pdf}
\caption{Visualization of CAM results of ToCo \cite{ru2023token} and our method MCC on MS COCO \emph{val} set. }
\label{fig:coco_cam_results}
\end{figure*}

==> sections/fig_coco_seg_results.tex <==
\begin{figure*}[!htb]
\centering
\includegraphics[width=0.85\linewidth,height=0.4\linewidth]{images/coco_seg_results.pdf}
\caption{Visualization of segmentation results of ToCo \cite{ru2023token} and our method MCC on MS COCO \emph{val} set. }
\label{fig:coco_seg_results}
\end{figure*}

==> sections/tab_block_mask.tex <==
\begin{table*}[!ht]
\begin{center}
\resizebox{0.95\linewidth}{!}{
    \begin{tabular}{c|p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering}}
    \hline
     
     Window Size &  $6 \times 6$ &  $8 \times 8$ & $9 \times 9$ & $10 \times 10$ & $11 \times 11$ & $12 \times 12$ \\
    \hline
    Seg & 64.2& 66.2 & 66.0 & 67.2 & 67.2 & 65.8  \\
    \hline
    \end{tabular}
}

\end{center}
\caption{Evaluation of Block Masking Strategy. The segmentation performance is evaluated on the PASCAL VOC \emph{val} set in terms of mIoU($\%$).}
\label{table:block_mask}
\end{table*}

% \resizebox{1.0\linewidth}{!}{
%     \begin{tabular}{c|p{0.9cm}<{\centering} p{1.1cm}<{\centering} p{1.1cm}<{\centering} p{1.1cm}<{\centering} p{1.1cm}<{\centering} p{1.1cm}<{\centering} | c c c c c c c c c c c c}
%     \hline
%      \multirow{2}*{Methods} & \multicolumn{6}{c|}{Block Masking} & \multicolumn{12}{c}{Random Masking}\\
%      ~ &  $6 \times 6$ &  $8 \times 8$ & $9 \times 9$ & $10 \times 10$ & $11 \times 11$ & $12 \times 12$ & s=1,2 & s=1,4 & s=1,7 & s=2,4 & s=2,7 & s=4,7 &  s=1,2,4 &  s=1,2,7  & s=1,4,7 & s=2,4,7 & s=1,2,4,7 & s=4 \\
%     \hline \hline
%     Seg & 64.2& 66.2 & 66.0 & 67.2 & 67.2 & 65.8 & 65.0 & 63.4 & 66.8 & 64.7 & 68.2 & 67.4 & 66.8 & 67.8 & 66.9 & 66.0 & 66.6 & 68.6  \\
%     \hline
%     \end{tabular}
% }

==> sections/tab_loss_weights.tex <==
\begin{table}[!ht]
\begin{center}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering}}
\hline
$\lambda_a$ & 0.1 & \textbf{0.2} & 0.3 & 0.5 \\
\hline 
Seg & 63.4 & \textbf{68.8} & 67.0 & 66.4 \\
\hline
\hline
$\lambda_m$ & 0.2 & \textbf{0.5} & 0.6 & 0.8 \\
\hline 
Seg & 67.2 & \textbf{68.8} & 67.7 & 66.4 \\
% \hline
% \hline
% $\lambda_3$ & 0.05 & \textbf{0.1} & 0.2 & 0.5 \\
% \hline 
% Seg & 67.0 & 68.8 & 66.0 & 63.3\\
\hline
\end{tabular}
}
\end{center}
\caption{Impact of loss weights $\lambda_a$ and $\lambda_m$. The performance is evaluated on the PASCAL VOC \textit{val} set in terms of mIoU($\%$).}
% yyf +only in train  upline
\label{table:loss_weights}
\end{table}

==> sections/tab_momentum.tex <==
\begin{table}[!ht]
\begin{center}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering}}
\hline
$m$ & 0.1 & 0.8 & \textbf{0.9} & 0.99 \\
\hline 
Seg &64.8 & 68.0 & \textbf{68.8} & 66.7\\
\hline
\end{tabular}
}
\end{center}
\caption{Impact of momentum $m$ in EMA. The performance is evaluated on the PASCAL VOC \textit{val} set in terms of mIoU($\%$).}
% yyf +only in train  upline
\label{table:momentum}
\end{table}

==> sections/tab_per_class.tex <==
\begin{table}[!ht]
\begin{center}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|c c c}
\hline
class & AFA & ToCo & MCC(Ours) \\
\hline \hline
bkg & 89.9 & 89.9 & \textbf{90.4}\\
aeroplane & 79.5 & \textbf{81.8} & 80.9\\
bicycle & 31.2 &35.4 & \textbf{37.9}\\
bird & \textbf{80.7} &68.1 & 79.0\\
boat & \textbf{67.2} & 62.0 & 63.4\\ 
bottle & 61.9 & 76.6 & \textbf{77.4}\\
bus & 81.4& \textbf{83.6} & 82.3\\
car & 65.4 &80.4 & \textbf{80.6}\\
cat & 82.3 & 87.7 & \textbf{88.8}\\
chair & \textbf{28.7} & 24.5 & 27.5\\ 
cow & 83.4 &\textbf{88.1} & 87.7\\
diningtable &41.6 & \textbf{54.9} & 49.7\\
dog & 82.2&\textbf{87.0} & 84.4\\
horse & 75.9 &\textbf{84.0} & 82.7\\
motorbike &70.2 & \textbf{76.0} & 74.2 \\
person &69.4&68.2 & \textbf{78.0}\\
pottedplant&53.0 &\textbf{ 65.6} & 62.1\\
sheep & 85.9&85.8 & \textbf{87.9}\\
sofa &\textbf{44.1} &42.4& 42.3\\
train & \textbf{64.2}&57.7 & 55.7\\
tvmonitor & 50.9&\textbf{65.6} & 62.3\\
\hline
mIOU & 66.0 &69.8 & \textbf{70.3}\\
\hline
\end{tabular}
}
\end{center}
\caption{Evaluation of the per-class semantic segmentation results in mIoU on the PASCAL VOC \textit{val} set}
% yyf +only in train  upline
\label{table:per_class}
\end{table}

==> sections/tab_pos_thres.tex <==
\begin{table}[!ht]
\begin{center}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering}}
\hline
$\mu$ & 0.1 & \textbf{0.2} & 0.3 & 0.4 \\
\hline 
Seg & 67.0 & \textbf{68.8} & 68.5 & 67.0 \\
\hline
\end{tabular}
}
\end{center}
\caption{Impact of threshold $\mu$ for positive/negative determination. The performance is evaluated on the PASCAL VOC \textit{val} set in terms of mIoU($\%$).}
% yyf +only in train  upline
\label{table:pos_thres}
\end{table}

==> sections/tab_random_mask.tex <==
\begin{table*}
\begin{center}
\resizebox{0.95\linewidth}{!}{
    \begin{tabular}{c|c c c c c c| c c c c| c}
    \hline
     Multi-scale &  1,2 & 1,4 & 1,7 & 2,4 & 2,7 & 4,7 &  1,2,4 &  1,2,7  & 1,4,7 & 2,4,7 & 1,2,4,7 \\
    \hline 
    Seg & 65.0 & 63.4 & 66.8 & 64.7 & 68.2 & 67.4 & 66.8 & 67.8 & 66.9 & 66.0 & 66.6  \\
    \hline
    \end{tabular}
}

\end{center}
\caption{Evaluation of Multi-scale Random Masking Strategy.  The segmentation performance is evaluated on the PASCAL VOC \emph{val} set in terms of mIoU($\%$).}
\label{table:mask}
\end{table*}

==> sections/tab_ratio_scale.tex <==
\begin{table}[htbp]
\begin{center}
\resizebox{1.0\linewidth}{!}{
    % \begin{tabular}{c|c|c|c|c}
    %     \hline
    %      HyperParam & s=1 & s=2 & \textbf{s=4} & s=7 \\
    %      \hline \hline
    %       r = 0.45  & 67.8 & 69.4 & 65.8 & 67.4 \\
    %       r = 0.50  & 66.7 & 67.5 & 69.5 & 67.2 \\
    %       r = 0.55  & 66.5 & 68.6 & 66.0 & 66.7 \\
    %       r = 0.60  & 66.1 & 66.8 & 69.7 & 67.2 \\
    %       r = 0.65  & 68.4 & 67.4 & 67.6 & 69.4 \\
    %       r = 0.70  & 68.0 & 69.2 & 68.5 & 68.4 \\
    %       r = 0.75  & 69.2 & 70.0 & 70.0 & 69.5 \\
    %       r = 0.80  & 68.6 & 69.8 & 67.6 & 68.7 \\
    %       r = 0.85  & 68.6 & 68.0 & 67.2 & 69.0 \\
    %       r = 0.90  & 67.4 & 69.4 & 68.7 & 69.6 \\
    %       \textbf{r = 0.95}  & 66.7 & 66.8 & \textbf{71.3} & - \\
    %       r = 0.99  & 66.7 & 69.1 & 69.2 & - \\
    %      \hline
    % \end{tabular}
    
    \begin{tabular}{c c|p{1.6cm}<{\centering}  p{1.6cm}<{\centering} p{1.6cm}<{\centering}  p{1.6cm}<{\centering}}
        \hline
         \multicolumn{2}{c|}{\multirow{2}*{HyperParam}} & \multicolumn{4}{c}{\textit{s}} \\
         ~ & ~ & 1 & 2 & \textbf{4} & 7 \\
         \hline \hline
          \multirow{12}*{\textit{r}} & 0.45  & 66.3 & 66.3 & 64.5 & 65.7 \\
          ~ & 0.50  & 64.6 & 65.0 & 67.0 & 65.7 \\
          ~ & 0.55  & 63.3 & 67.2 & 65.3 & 64.9 \\
          ~ & 0.60  & 63.7 & 64.2 & 67.0 & 65.4 \\
          ~ & 0.65  & 65.9 & 65.8 & 65.8 & 66.8 \\
          ~ & 0.70  & 65.2 & 66.6 & 66.5 & 66.1 \\
          ~ & 0.75  & 67.1 & 68.4 & 67.6 & 66.8 \\
          ~ & 0.80  & 66.2 & 66.4 & 66.0 & 66.2 \\
          ~ & 0.85  & 66.3 & 65.7 & 65.3 & 65.4 \\
          ~ & 0.90  & 65.1 & 67.5 & 66.8 & 67.1 \\
          ~ & \textbf{0.95}  & 64.6 & 65.1 & \textbf{68.6} & - \\
          ~ & 0.99  & 64.6 & 65.1 & 67.1 & - \\
         \hline
    \end{tabular}
}
\end{center}
\caption{Ablation Study on random masking under varying the mask ratios and scales. \textit{s} stands for scale and \textit{r} represents mask ratio. The segmentation results are reported from VOC \emph{val} set in terms of mIoU($\%$).}
\label{table:abl_mask}
\end{table}


==> sections/tab_temp.tex <==
\begin{table}[!ht]
\begin{center}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering} p{1.6cm}<{\centering}}
\hline
$\tau$ & 0.1 & 0.2 & \textbf{0.5} & 0.8 \\
\hline 
Seg & 67.7& 67.9 & \textbf{68.8} & 66.7\\
\hline
\end{tabular}
}
\end{center}
\caption{Impact of temperature $\tau$ in contrastive loss. The performance is evaluated on the PASCAL VOC \textit{val} set in terms of mIoU($\%$).}
% yyf +only in train  upline
\label{table:temp}
\end{table}
